Robust Impulse Responses using External Instruments: the Role of Information

External-instrument identification leads to biased responses when the shock is not invertible and the measurement error is present. We propose to use this identification strategy in a structural Dynamic Factor Model, which we call Proxy DFM. In a simulation analysis, we show that the Proxy DFM always successfully retrieves the true impulse responses, while the Proxy SVAR systematically fails to do so when the model is either misspecified, does not include all relevant information, or the measurement error is present. In an application to US monetary policy, the Proxy DFM shows that a tightening shock is unequivocally contractionary, with deteriorations in domestic demand, labor, credit, housing, exchange, and financial markets. This holds true for all raw instruments available in the literature. The variance decomposition analysis highlights the importance of monetary policy shocks in explaining economic fluctuations, albeit at different horizons.

==> inputs/frob.tex <==
\begin{tabular}{lcc}
\hline\hline
&\textbf{Shock}&\textbf{IRF}\\\hline\hline
\textbf{Proxy VAR}&100.00&100.00\\
\textbf{Proxy FAVAR}&20.72&16.56\\
\textbf{Proxy DFM}&17.95&15.07\\
\textbf{Proxy VAR}&100.00&100.00\\
\textbf{Proxy FAVAR}&31.19&20.94\\
\textbf{Proxy DFM}&19.86&16.04\\
\textbf{Proxy VAR}&100.00&100.00\\
\textbf{Proxy FAVAR}&39.85&23.47\\
\textbf{Proxy DFM}&23.90&17.94\\
\hline
\hline
\end{tabular}


==> inputs/frob_NFF.tex <==
\begin{tabular}{lcc}
\hline\hline
&\textbf{Shock}&\textbf{IRF}\\\hline\hline
\textbf{Proxy VAR}&100.00&100.00\\
\textbf{Proxy FAVAR}&99.34&130.72\\
\textbf{Proxy DFM}&102.48&130.61\\
\textbf{Proxy VAR}&100.00&100.00\\
\textbf{Proxy FAVAR}&60.10&77.43\\
\textbf{Proxy DFM}&57.08&73.40\\
\textbf{Proxy VAR}&100.00&100.00\\
\textbf{Proxy FAVAR}&53.99&53.66\\
\textbf{Proxy DFM}&44.52&47.71\\
\hline
\hline
\end{tabular}


==> inputs/fundtest_empi.tex <==
\begin{tabular}{lccccc}
\hline\hline
&\textbf{1}&\textbf{2}&\textbf{3}&\textbf{4}&\textbf{5}\\\hline\hline
\textbf{VAR    1%}&0.00&0.00&0.00&0.00&4.17\\
\textbf{VAR    5%}&2.08&0.00&1.04&4.17&12.50\\
\textbf{VAR    10%}&10.42&2.08&5.21&11.46&22.92\\
\textbf{FAVAR  1%}&0.00&0.00&0.00&0.00&0.00\\
\textbf{FAVAR  5%}&0.00&0.00&0.00&0.00&5.21\\
\textbf{FAVAR  10%}&1.04&1.04&0.00&6.25&11.46\\
\textbf{DFM    1%}&0.00&0.00&0.00&0.00&0.00\\
\textbf{DFM    5%}&0.00&0.00&0.00&0.00&0.00\\
\textbf{DFM    10%}&0.00&0.00&0.00&0.00&0.00\\
\hline
\hline
\end{tabular}

